LOGAN: High-Performance GPU-Based X-Drop Long-Read Alignment

Pairwise sequence alignment is one of the most computationally intensive kernels in genomic data analysis, accounting for more than 90% of the runtime for key bioinformatics applications. This method is particularly expensive for third-generation sequences due to the high computational cost of analyzing sequences of length between 1Kb and 1Mb. Given the quadratic overhead of exact pairwise algorithms for long alignments, the community primarily relies on approximate algorithms that search only for high-quality alignments and stop early when one is not found. In this work, we present the first GPU optimization of the popular X-drop alignment algorithm, that we named LOGAN. Results show that our high-performance multi-GPU implementation achieves up to 181.6 GCUPS and speed-ups up to 6.6x and 30.7x using 1 and 6 NVIDIA Tesla V100, respectively, over the state-of-the-art software running on two IBM Power9 processors using 168 CPU threads, with equivalent accuracy. We also demonstrate a 2.3x LOGAN speed-up versus ksw2, a state-of-art vectorized algorithm for sequence alignment implemented in minimap2, a long-read mapping software. To highlight the impact of our work on a real-world application, we couple LOGAN with a many-to-many long-read alignment software called BELLA, and demonstrate that our implementation improves the overall BELLA runtime by up to 10.6x. Finally, we adapt the Roofline model for LOGAN and demonstrate that our implementation is near-optimal on the NVIDIA Tesla V100s.

==> tables/tab2.tex <==
\begin{table}[t]

	\centering
	\caption{Execution times on ``POWER9'' platform with 6 NVIDIA Tesla V100s in seconds for 3.62M alignments ({\em A. baumannii}).\newline
	\textbf{BELLA} indicates the original software, while \textbf{LOGAN} indicates that BELLA uses LOGAN for alignment.}
	\label{table:performance_comparison_2}
	\resizebox{\columnwidth}{!}{%
\begin{tabular}{rrrrrr}
	\toprule
		\multirow{2}{*}{\textbf{$X$-Drop}} &\textbf{BELLA}& \textbf{LOGAN} & \textbf{LOGAN} & \textbf{Speed-Up}& \textbf{Speed-Up}\\
		 &\textbf{168 CPU Threads}& \textbf{1 GPU} & \textbf{6 GPU} & \textbf{1 GPU} & \textbf{6 GPU} \\
	\midrule
	    5 &  52.20 & 123.12 & 109.81 & 0.4$\times$ & 0.5$\times$ \\ 
	\midrule
        10 & 106.55 & 129.07 & 111.01 & 0.8$\times$ & 1.0$\times$ \\ 
    \midrule
        15 & 170.43 & 135.48 & 113.18 & 1.3$\times$ & 1.5$\times$ \\ 
    \midrule
        20 & 222.34 & 142.39 & 114.90 & 1.6$\times$ & 1.9$\times$ \\ 
    \midrule
        25 & 270.02 & 149.87 & 116.92 & 1.8$\times$ & 2.3$\times$ \\  
    \midrule
        30 & 309.54 & 157.93 & 117.27 & 2.0$\times$ & 2.6$\times$ \\  
    \midrule
        35 & 346.35 & 166.65 & 119.51 & 2.1$\times$ & 2.9$\times$ \\  
    \midrule
        40 & 379.67 & 176.06 & 121.38 & 2.2$\times$ & 3.1$\times$ \\ 
    \midrule
        50 & 440.45 & 186.23 & 122.25 & 2.4$\times$ & 3.6$\times$ \\ 
    \midrule
        80 & 584.32 & 197.20 & 124.79 & 3.0$\times$ & 4.7$\times$ \\
    \midrule
        100 & 666.11 & 219.75 & 126.74 & 3.0$\times$ & 5.3$\times$ \\
	\bottomrule
	\end{tabular}%
	}
\end{table}
